One-level density of the family of twists of an elliptic curve over function fields

We fix an elliptic curve $E/\mathbb{F}_q(t)$ and consider the family $\{E\otimes\chi_D\}$ of $E$ twisted by quadratic Dirichlet characters. The one-level density of their $L$-functions is shown to follow orthogonal symmetry for test functions with Fourier transform supported inside $(-1,1)$. As an application, we obtain an upper bound of 3/2 on the average analytic rank. By splitting the family according to the sign of the functional equation, we obtain that at least $12.5\%$ of the family have rank zero, and at least $37.5\%$ have rank one. The Katz and Sarnak philosophy predicts that those percentages should both be $50\%$ and that the average analytic rank should be $1/2$. We finish by computing the one-level density of $E$ twisted by Dirichlet characters of order $\ell\neq 2$ coprime to $q$. We obtain a restriction of $(-1/2,1/2)$ on the support with a unitary symmetry.

==> Introduction.tex <==
\section{Introduction}
We study the one-level density of the family of twists of an elliptic curve defined over $\mathbb{F}_q(t)$. Over $\mathbb{Q}$, the one-level density of this family was studied by Heath-Brown \cite{heath-brown:2003} for quadratic twists. The first results obtained in the present paper are analogous to what he obtained. Under a hypothesis slightly stronger than the Riemann Hypothesis for elliptic curves, Fiorilli \cite{Fiorilli:2014} showed that the average analytic rank of this family is exactly $1/2$. For cubic Dirichlet $L$-functions over $\mathbb{Q}$, Cho and Park \cite{chopark:2017} computed the one-level density and obtained the restriction of $(-1,1)$ on the support of the test functions along with a unitary symmetry. They also computed \cite{CHO2019139} the $n$-level densities for the family of cubic twists of any given cuspidal representation of $\text{GL}_m(A_\mathbb{Q})$, and they showed that the symmetry is unitary.  Over cubic Galois number fields, Meisner \cite{meisner:2017} computed the one-level density of the associated $L$-functions and showed that the symmetry is unitary with a restriction of $(-1/2,1/2)$ on the support. For the one-level density of Dirichlet $L$-functions of order $r$ over $\mathbb{Q}$, Cho and Park \cite{chopark2:2019} showed that the symmetry is unitary, and obtained the restriction of (-1,1) on the support. They also obtained the restriction of $(-1/m,1/m)$ on the support for the family of twists of order $r$ of any given cuspidal representation of $\text{GL}_m(A_\mathbb{Q})$. All of the above results are under the Generalized Riemann Hypothesis. Over function fields, results are unconditional since the Weil's conjectures has been proved.\\ \\
Over $\mathbb{F}_q(t)$, the one-level density of the family of quadratic Dirichlet $L$-functions was studied by Rudnick \cite{Rudnick:2008} where he obtained a restriction of $(-2,2)$ on the support, with a symplectic symmetry. Under further restrictions on the support, Bui and Florea \cite{Bui&Florea:2016} were able to compute lower order terms for the one-level density of this family. The first four moments of this family were obtained by Florea \cite{florea2015second},  \cite{florea2016fourth}. For cubic Dirichlet $L$-functions over $\mathbb{F}_q(t)$, David, Florea, and Lalín \cite{David&Florea&Lalin:2019} computed the mean values of the $L$-functions. They also proved that a positive proportion of these $L$-functions do not vanish at the central point \cite{chantal2:2020}. For twists of order $r$ such that $q\equiv 1$ mod $r$, Meisner determined the number of $\mathbb{F}_q$-points of the associated curves \cite{meisner:2015}. \\ \\
Throughout this paper, a prime $p\neq 2,3$ is fixed and we fix $q=p^n$ for any integer $n\geq1$. We also fix an elliptic curve $E:y^2=x^3+Ax+B$ over $\mathbb{F}_q[t]$ under its minimal Weierstrass model such that it has at least one prime of multiplicative reduction, has additive reduction at infinity, and such that its $j$-invariant isn't zero (see \cite{silverman:2009} for background). We write $A$ instead of $A(t)$ for elements of $\mathbb{F}_q[t]$. The conductor of $E$ is denoted by $N_E$.\\ \\
Let $\mathcal{M}_N\subset\mathbb{F}_q[t]$ be the set of monic polynomials of degree $N$ and let $\mathcal{H}_{N,C}\subset\mathcal{M}_N$ be the set of square-free polynomials of degree $N$ congruent to $C$ modulo $N_E$ where $C$ is coprime to $N_E$. We denote by $\mathcal{H}^*_N$ the set of square-free polynomials of degree $N$ that are coprime to $N_E$. In particular, we have the partition $\mathcal{H}_N^* = \bigcup_{\substack{C \text{ mod } N_E\\(C,N_E)=1}} \mathcal{H}_{N,C}$.
The main family of this paper is the set of quadratic twists of $E$. Each twist of $E$  is denoted by $E\otimes\chi_D$ where $\chi_D$ is the unique quadratic Dirichlet character of conductor $D$, where $D\in\mathcal{H}^*_N$. To each twist is associated a unitary matrix (up to conjugacy class) called the Frobenius of $E\otimes\chi_D$ denoted by
\begin{equation}\label{matrix}
 \Theta_D = \left(\begin{matrix}e^{i\theta_{D,1}} & & \\ & \ddots & \\ & & e^{i\theta_{D,M}}\end{matrix}\right)
 \end{equation}
 where the  $e^{i\theta_{D,j}}$ are called the Frobenius eigenvalues of $E\otimes\chi_D$ and $0 \leq \theta_{D,j} < 2\pi$.
 The average of traces of powers of $\Theta_D$ over $\mathcal{H}_{N,C}$ is defined by
\[ \langle\text{tr } \Theta^n\rangle_{N,C} := \frac{1}{|\mathcal{H}_{N,C}|}\sum_{D \in \mathcal{H}_{N,C}} \sum_{j=1}^{M} e^{in\theta_{D,j}}. \]
We prove the following.
\begin{theorem}\label{thm:main}
For $\epsilon>0$, $n>0$, and $N>4\,\emph{deg}(N_E)$
\begin{align*}
\langle\emph{tr } \Theta^n\rangle_{N,C} &=
\begin{cases}
 1, & \emph{if } n \emph{ is even} \\
 0, & \emph{if } n \emph{ is odd}
  \end{cases} \\
  &+\mathcal{O}_{E,q}\left((n+N)N^{2\,\emph{deg}(N_E)+3}\left( \frac{1}{q^{N/8}} + \frac{1}{q^{\epsilon N}} + \frac{q^{n/2}}{q^{(1-\epsilon)N}}\right) +  n^2q^{-n/4} \right).
\end{align*}
\end{theorem}
This is in agreement with the mean values over $O(M)$ given in \cite{Diaconis&Shahshahani:1994}
\begin{equation}\label{eq:ortho}
\int_{O(M)} \text{tr } \Theta^n d\Theta=
\begin{cases}
 1, & \text{if }n \text{ is even} \\
 0, & \text{if } n \text{ is odd}
  \end{cases}
\end{equation}
 with respect to the Haar measure where $O(M)$ is the orthogonal group of dimension $M$. \\ \\
 As an application we compute the one-level density of the family. The Schwartz space $\mathcal{S}(\mathbb{R})$ is a space of rapidly decreasing functions on $\mathbb{R}$ and is defined by
\[ \mathcal{S}(\mathbb{R}) := \{f \in C^\infty(\mathbb{R}) \, | \, \forall \alpha,\beta \in \mathbb{N}, \Vert f \Vert_{\alpha,\beta} < \infty\}  \text{ where } \Vert f \Vert_{\alpha,\beta} := \text{sup}_{x \in \mathbb{R}} | x^\alpha f^{(\beta)}(x)|.\]
For an even function $\phi \in \mathcal{S}(\mathbb{R})$ and $M\geq 0$, we define
\[ F(\theta):=\sum_{k\in\mathbb{Z}} \phi \left(M \left(\frac{\theta}{2\pi}-k\right)\right)\]
which has period $2\pi$ and is localized on an interval of size $\approx 1/M$ around 0 in $\mathbb{R}/2\pi\mathbb{Z}$. Let $\Theta$ be an $M \times M$ matrix with eigenvalues $e^{i\theta_j}$, where $0\leq \theta_j<2\pi$. We define 
\[ Z_{\phi}(\Theta):=\sum_{j=1}^M F(\theta_j).\]
The one-level density of the family $\mathcal{H}_{N,C}$ is the average
\[ \langle Z_{\phi}\rangle_{N,C}:= \frac{1}{|\mathcal{H}_{N,C}|} \sum_{D \in \mathcal{H}_{N,C}} Z_{\phi} (\Theta_D) \]
where $\Theta_D$ is given by (\ref{matrix}). The one-level density picks up the $\theta_j$ near 0 and it reveals the symmetry type of our family. We prove the following result on the one-level density.
\begin{customcor}{\ref{cor:1ld}}
For $\phi \in \mathcal{S}(\mathbb{R})$ an even function such that \emph{supp}$(\hat{\phi})\subset (-1,1)$, we have for the one-level density of the family of quadratic twists of $E$
\[ \langle Z_{\phi}\rangle_{N,C}=\int_{O(M)} Z_{\phi}(\Theta) d\Theta + \mathcal{O}_{E,q}(1/N)\]
where $M=2N+\emph{deg}(N_E)-4$.
\end{customcor}
As an application, we get an upper bound on the average analytic rank. The analytic rank of $E\otimes\chi_D$ is defined as the number of $\theta_{D,j}=0$ in $\Theta_D$, and we denote it by $r(E\otimes\chi_D)$. We define
\[ \langle r \rangle_{N,C} := \frac{1}{|\mathcal{H}_{N,C}|} \sum_{D \in \mathcal{H}_{N,C}} r(E\otimes\chi_D)\]
and the average analytic rank is defined as
\[ r_C := \lim_{N\rightarrow \infty} \langle r \rangle_{N,C}  \]
if the limit exists. We prove the followings.
\begin{customthm}{\ref{thm:rank}}
We have $r_C \leq 3/2$.
\end{customthm}
In particular, the average analytic rank is $\leq 3/2$ in the whole family of twists $D\in\mathcal{H}_{N}^*$. By splitting the family according to congruence classes we get the following result on the non-vanishing at the central point.
\begin{customthm}{\ref{thm:nv}}
At least $12.5\%$ of the family of quadratic twists of $E$ have rank zero and at least $37.5\%$ have rank one as $N\rightarrow \infty$.
\end{customthm}
In the final section, we study the one-level density for the family of twists of $E$ of order $\ell$ coprime to $q$. However, the results are too weak to produce any significant bound on the average analytic rank. We get the following restriction on the support of the Fourier transform of $\phi$ where $U(M)$ is the unitary group of dimension $M$.
\begin{customthm}{\ref{thm:ao}}
For $\phi \in \mathcal{S}(\mathbb{R})$ an even function such that \emph{supp}$(\hat{\phi})\subset (-1/2,1/2)$, we have for the one-level density of the family of twists of $E$ of order $\ell\neq 2$ and $(\ell,q)=1$
\[ \langle Z_{\phi}\rangle_{N,C}=\int_{U(M)} Z_{\phi}(\Theta) d\Theta + \mathcal{O}_{E,q,\ell}(1/N)\]
where $M=2N+\emph{deg}(N_E)-4$.
 \end{customthm}
The condition supp$(\hat{\phi})\subset (-1/2,1/2)$ for twists of $E$ is the analogous result of the condition supp$(\hat{\phi})\subset (-1/m,1/m)$ for twists of a given cuspidal representation of $\text{GL}_m(A_\mathbb{Q})$ obtained by Cho and Park over $\mathbb{Q}$ \cite{chopark2:2019}.
